Unbalanced Optimal Transport: A Unified Framework for Object Detection

During training, supervised object detection tries to correctly match the predicted bounding boxes and associated classification scores to the ground truth. This is essential to determine which predictions are to be pushed towards which solutions, or to be discarded. Popular matching strategies include matching to the closest ground truth box (mostly used in combination with anchors), or matching via the Hungarian algorithm (mostly used in anchor-free methods). Each of these strategies comes with its own properties, underlying losses, and heuristics. We show how Unbalanced Optimal Transport unifies these different approaches and opens a whole continuum of methods in between. This allows for a finer selection of the desired properties. Experimentally, we show that training an object detection model with Unbalanced Optimal Transport is able to reach the state-of-the-art both in terms of Average Precision and Average Recall as well as to provide a faster initial convergence. The approach is well suited for GPU implementation, which proves to be an advantage for large-scale models.

==> arch/old.tex <==
% \section{Optimal Transport \& Further Connections}

% \subsection{Balanced Optimal Transport}

% \subsection{Unbalanced Optimal Transport}


% We will now consider the case of unbalanced optimal transport. We first recall the Kullback-Leibler divergence.
% \begin{definition}
%     The Kullback-Leibler divergence between two atomic measures of same size $\bm{\mu}, \bm{\nu} \in \mathbb{R}_+^m$ is given by
%     \begin{equation}
%         \mathrm{KL}(\bm{\mu} |\bm{\nu}) = \sum_{i=1}^m \mu_i \log \left( \frac{\mu_i}{\nu_i}\right).
%     \end{equation}
% \end{definition}
% It is often also called the \emph{relative entropy} and behaves like a distance but is not metric as it does not satisfy the symmetry property, nor the triangular inequality. We can now define the unbalanced Wasserstein distance.
% \begin{definition}
% The unbalanced Wasserstein distance between two atomic measures $\bm{\mu} \in \mathbb{R}_+^m$ and $\bm{\nu} \in \mathbb{R}_+^n$, a cost matrix $\bm{C} \in \mathbb{R}_+^{m \times n}$ and parameters $\tau_1 \in \mathbb{R}_+$ and $\tau_2 \in \mathbb{R}_+$ is given by
% \begin{equation}
% \label{eq:unbalanced}
% \begin{array}{rcl}
% \displaystyle
%     \mathcal{W}_{\tau_1, \tau_2}(\bm{\mu},\bm{\nu}) = \hspace{-.5em}\min_{\bm{P} \in \mathbb{R}_+^{m \times n}} \hspace{-.3em}\langle \bm{P}, \bm{C} \rangle \hspace{-.7em}&+&\hspace{-.7em} \tau_1 \mathrm{KL}\left(\left. \bm{P}1^\top\right| \bm{\mu} \right)\\
%     &+&\hspace{-.7em} \tau_2 \mathrm{KL}\left( \bm{P}1\left| \bm{\nu} \right.\right).
% \end{array}
% \end{equation}
% \end{definition}

% \subsubsection{Limit Cases}
% We can already observe that the case $\tau_1 = \tau_2 = 0$ is degenerate and $\mathcal{W}_{0,0}(\bm{\mu},\bm{\nu}) = 0$. In the limit towards infinity, we retrieve back the original optimal transport problem.
% \begin{proposition}
% Given two atomic measures $\bm{\mu} \in \mathbb{R}_+^m$ and $\bm{\nu} \in \mathbb{R}_+^n$, we have
% \begin{equation}
%     \lim_{\substack{\tau_1 \to \infty \\ \tau_2 \to \infty}}\underset{\bm{P} \in \mathbb{R}_+^{m \times n}}{\operatorname{min}} \mathcal{W}_{\tau_1, \tau_2}(\bm{\mu},\bm{\nu}) = \mathcal{W}(\bm{\mu},\bm{\nu}).
% \end{equation}
% \end{proposition}
% \begin{proof}
% This corresponds to changing the two divergence terms to strict equality constraints, which corresponds to the original Wasserstein distance. For a more rigorous proof, we refer to [Chizat...].
% \end{proof}
% We finally have to discuss the mixed limit case.

% \paragraph{Minimum}
% We can show a connection between a minimum and the unbalanced optimal transport problem. By taking the limit case of Eq.~\ref{eq:unbalanced} with $\tau_1 \to 0$ and $\tau_2 \to \infty $. More formally, we can state the following proposition.
% \begin{proposition}
% \label{unbalanced_limit}
% Given any source $\bm{\mu} \in \mathbb{R}^m$, a target $\bm{\nu} = \left\{a\right\}^n$ with $\alpha \in \mathbb{R}_+$ and a cost matrix $\bm{C} \in \mathbb{R}_+^{m \times n}$, the coupling $\bm{P} \in \left\{0,\alpha\right\}_+^{m \times n}$ given by
% \begin{equation}
%    \bm{P} =  \lim_{\substack{\tau_1 \to 0 \\ \tau_2 \to \infty}}\underset{\bm{P} \in \mathbb{R}_+^{m \times n}}{\operatorname{argmin}} \mathcal{W}_{\tau_1, \tau_2}(\bm{\mu},\bm{\nu}),
% \end{equation}
% returns the minimum for each target. More specifically
% \begin{equation}
%     \bm{P}_{ij} = 
%     \begin{cases}
%     \alpha, \quad \text{if $\bm{C}_{ij} = \min_k \bm{C}_{kj} $}, \\
%     0, \quad \text{otherwise}.
%     \end{cases}
% \end{equation}
% \end{proposition}
% \begin{proof}
% Informally, in the limit $\tau_1 \to 0$, there will be no consideration for how the final distribution of $\bm{\mu}$ will look like (hence its non-specification in the proposition). Conversely, in the limit $\tau_2 \to \infty$ will strictly require that $\bm{P}1 = \bm{\nu}$. In other words, we have the constrained problem
% \begin{equation}
%     \begin{array}{rl}
%     \displaystyle
%        \min_{\bm{P} \in \mathbb{R}_+^{m \times n}} & \langle \bm{P}, \bm{C} \rangle,\\
%         \mathrm{s.t.} & \sum_i\bm{P}_{ij} = \alpha \qquad \text{for each $j$}. 
%     \end{array}
% \end{equation}
% It is clear (??) that the optimal solution is given by the minimum for each target.
% \end{proof}
% By symmetry, the converse case with $\tau_1 \to \infty$ and $\tau_2 \to 0$ is equivalent to \cref{unbalanced_limit} where the source and the target are exchanged. In other words, the minimum is taken row-wise of $\bm{C}$ instead of column-wise.

% \subsection{Approximation of the Hungarian Algorithm}
% The idea is to keep $\tau_2 \to \infty$ and search for a proper $\tau_1$ approximating the Hungarian algorithm. Indeed, in one limit we retrieve the original optimal transport case, which corresponds to finding the source minimizing the cost with each target disregarding the fact that a same source may be assigned to multiple targets. In the other limit, we retrieve the original optimal transport problem, which corresponds to finding the optimal match where the mass of each source is conserved, leading to a very spread out match.

% There must be a $\tau_2$ which gives good compromise. I believe there is no strict equivalence between the Hungarian algorithm and unbalanced optimal transport. More rigorously, no $\tau_1$ exists such that the unbalanced optimal transport solution strictly corresponds to the solution of the Hungarian algorithm. A first idea would be to prove that with a counter-example.

% \subsubsection{One Target}
% This case will lead to the solution of the Hungarian algorithm, because the minimum also corresponds. In other words, there is no lower bound for $\tau_1$.

% Lets us first consider the unbalances case where we have $n$ different sources and only one target. The cost matrix and the matching matrix are then reduced to vectors $c_i$ and $p_i$.

% We can first show that the solution corresponding to optimal matching \emph{(without regularization)} would equal
% \begin{equation}
%     \frac1n \sum_i c_i,
% \end{equation}
% and the solution where only the minimum is matched is equal to
% \begin{equation}
%     c_k + \tau_1 \log m.
% \end{equation}
% In order to guarantee that minimum matching is smaller that the normal problem, we must guarantee that $\tau_1 \leq \tau_{\mathrm{max}}$ with
% \begin{equation}
%     \tau_{\mathrm{max}} = \frac{1}{n \log n}\sum_i c_i - \frac{c_k}{\log n},
% \end{equation}
% where $k$ corresponds to the optimal matching. This is however not sufficient. If we can guarantee that the solution is smaller than the limit case for $\tau \mapsto \infty$, we didn't prove that no intermediate solution doesn't exist between both. Proving further (by looking at the Hessian because of the convexity e.g.) seems to be a difficult problem (and of course depends on the cost).

% A few results to play with:
% \begin{equation}
%     \frac{\partial W(a,b)}{\partial p_{ij}} = c_{ij} + \log \left( m \sum_i p_{ij} \right) + \frac{p_{ij}}{\sum_i p_{ij}}.
% \end{equation}

% \subsubsection{General Case}
% We now consider the case with $n$ sources and $m$ targets. The cost of the hungarian mapping would be
% \begin{equation}
%     \frac1m \sum c_{\mathrm{opt}} + \tau\log \left( \frac mn \right)
% \end{equation}


% Idea: The cost of wanting a Hungarian-type matching is $\tau\log \left( \frac mn \right)$. We have to guarantee that the "mapping" cost is greater.
% A solution heuristic for the choice of $\tau$ would be to consider two limit cases. The one where we take the minimum for all elements per target (a perfect match but considering two sources may be mapped to the same target) and the one where we take the mean (where $p_{ij} = \frac{1}{\max (m,n)}$). In other words $\tau \leq \tau_0$ with
% \begin{equation}
% \tau_0 = \frac{\Delta}{\log (m / n)}.    
% \end{equation} 
% This is an sub-optimal result, but at least it is (easily) provable.

% Note: by sparsifying the matching matrix $\bm{P}$, we will go towards more numerical unstability.

% Note 2: I may have exchanged $m$ and $n$ above. When deciding on the theoretical trajectory, that has of course to be all rigourified.

\subsubsection{A lower bounds}
Let us consider the cost matrix
\begin{equation}
    \bm{C} = \left(
    \begin{array}{cc}
       c_2  &  c_2+c_1\\
        c_1 & c_1 \\
        c_3 + c_1 & c_3\end{array}\right),
\end{equation}
with $c_1 < c_2 < c_3$. 

\paragraph{Hungarian}
The solution to the Hungarian algorithm is given by
\begin{equation}
    \bm{C} = \left(
    \begin{array}{cc}
        \frac12  & 0 \\
        0 & \frac12 \\
        0 & 0
    \end{array}\right),
\end{equation}
The cost is given by
\begin{equation}
    \frac12(c_1 + c_2) + \tau_1 \log \frac32
\end{equation}
\paragraph{Minimum}
and to the minimum match
\begin{equation}
    \bm{C} = \left(
    \begin{array}{cc}
        0 & 0 \\
        \frac12 & \frac12 \\
        0 & 0
    \end{array}\right),
\end{equation}
The solution is given by
\begin{equation}
    c_1 + \tau_1 \log 3.
\end{equation}
In other words, the cost of the Hungarian algorithm is smaller that the minimum if
\begin{equation}
    \tau > \frac{1}{2 \log 2}\left(c_2-c_1\right)
\end{equation}

\subsubsection{A Condition for Optimality}
An optimality condition could be $$\frac{\partial f_\tau}{\partial \bm{P}} = 0.$$ It seems that this can only be satisfied if $m=n$ (same number of source and target) and $\tau_1 \to \infty$, which is the already known case.

The choice of $\tau_1$ is thus the core of the problem here. If it is too small, we risk having the same source matched to multiple targets (which is mitigated in practice by augmenting the number of sources). If it is too big, we risk of not specifically favoring a specific source (is that a problem if we take the max?? back to beginning then). To summarize, $\tau_1$ is a trade-off parameter to favor specificity or not.

==> arch/old_abstract.tex <==
\begin{abstract}
A key difficulty in the training of supervised object detection models is the correct matching of the predicted bounding boxes to their ground truth. Solutions up to now consisted either in an overspecification of the number of predicted bounding boxes, either in greedy algorithms. In this paper, we propose a novel method based on optimal transport. A theoretical development is then backed by experimental data, illustrating that our method beats the state-of-the-art both in inference and speed, on toy examples and large-scale datasets.
\end{abstract}

==> arch/related.tex <==
\section{Related Work}

In general, box-based object detection models consist in predicting, for each image, a set of boxes. These boxes are described by a position and vector encoding the probability for each class. Training consists in minimizing  a loss $\mathcal{L} = \mathcal{L}_{\text{localization}} + \mathcal{L}_{\text{classification}}$, where the first term consists in matching the positions of the predicted boxes to the correct target positions. The second term matches the corresponding classifications.

The main difficulty relies in insuring that each target box is assigned to one predicted box with corresponding class, at least during the inference. All the other predicted boxes should be matched to a default \emph{no-object} class, often referred to as \emph{background}. To guarantee this unique matching, many solutions have been proposed. 

[YOLO] for example predicts way too much boxes, many being matched towards the same target. During inference, the different overlapping predicted boxes with similar class predictions are then reduced to one by maximizing a confidence score. This mechanism is called \emph{Non-Maximal Suppression}.

[DETR] alternatively works by guaranteeing a unique match during training. This is done by using the \emph{Hungarian} algorithm, on a specific loss 

\paragraph{One-stage Object Detectors}

\paragraph{DETR}

...

\iffalse
DETR computes a minimal cost bipartite matching between predicted and ground truth objects.
\begin{equation*}
    \hat{\sigma}=\underset{\sigma \in \mathfrak{S}_{N}}{\arg \min } \sum_{i}^{N} \mathcal{L}_{\operatorname{match}}\left(y_{i}, \hat{y}_{\sigma(i)}\right)
\end{equation*}
This optimal assignment is computed with the Hungarian algorithm.
\else

\paragraph{Optimal Transport in Computer Vision}
